Analysis of a cusped helicon plasma thruster discharge

A compact helicon plasma thruster that features a cusp in its internal magnetic field is analyzed with experiments and simulations. A compensated Langmuir probe and a Faraday cup are used in the former, while a hybrid PIC/fluid transport model combined with a frequency-domain electromagnetic field model are used in the latter. Measurements serve to tune the anomalous transport parameters of the model and overall show the same trends as the numerical results, including a secondary peak of electron temperature downstream in the magnetic nozzle, where electron cyclotron resonance conditions for the 13.56 MHz excitation frequency are met. The cusp plays a central role in determining the plasma losses to the walls and the profile of electron temperature, which in turn defines the excitation and ionization losses. While losses to the rear wall are reduced, losses to the lateral wall are increased, which, together with the low production efficiency, limit the performance of the device. Shorter chamber lengths and optimization of antenna and cusp location are suggested as potential ways to improve performance.

==> recortes.tex <==
Interestingly, the peak of electron temperature at the source is found away from the axis and we observe a clear separation between the cold plasma upstream the singular point and the warm plasma downstream. 



The lack of neutral depletion near the axis, as expected in \cite{zhou19a}, indicates that ionization rate is not large at the axis. This is further hinted at by the power deposition profile \ref{fig:power}. 

